Path Integral Particle Filtering for Hybrid Systems via Saltation Matrices

State estimation for hybrid systems that undergo intermittent contact with their environments, such as extraplanetary robots and satellites undergoing docking operations, is difficult due to the discrete uncertainty propagation during contact. To handle this propagation, this paper presents an optimal-control-based particle filtering method that leverages saltation matrices to map out uncertainty propagation during contact events. By exploiting a path integral filtering framework that exploits the duality between smoothing and optimal control, the resulting state estimation algorithm is robust to outlier effects, flexible to non-Gaussian noise distributions, and handles challenging contact dynamics in hybrid systems. To evaluate the validity and consistency of the proposed approach, this paper tests it against strong baselines on the stochastic dynamics generated by a bouncing ball and spring loaded inverted pendulum.

==> final_paper/contributions.tex <==
\section{Contributions}
Karthik Shaji wrote the optimal control methodology, developed the algorithm structure, did the mathematical derivations for this paper, and wrote the majority of this paper. Sreeranj Jayadevan handled the hybrid systems dynamics, integrations, and reference extensions. Bo Yuan and Hongzhe Yu provided advisory contributions on the particle filter derivations and the stochastic hybrid dynamics, helping lay out the design of the algorithm. Professor Chen supervised 

% Add Prof. Chen and get his approval of what to say "supervisory"
